Performance Analysis of the IEEE 802.11e Enhanced Distributed Coordination Function using Cycle Time Approach

The recently ratified IEEE 802.11e standard defines the Enhanced Distributed Channel Access (EDCA) function for Quality-of-Service (QoS) provisioning in the Wireless Local Area Networks (WLANs). The EDCA uses Carrier Sense Multiple Access with Collision Avoidance (CSMA/CA) and slotted Binary Exponential Backoff (BEB) mechanism. We present a simple mathematical analysis framework for the EDCA function. Our analysis considers the fact that the distributed random access systems exhibit cyclic behavior where each station successfully transmits a packet in a cycle. Our analysis shows that an AC-specific cycle time exists for the EDCA function. Validating the theoretical results via simulations, we show that the proposed analysis accurately captures EDCA saturation performance in terms of average throughput, medium access delay, and packet loss ratio. The cycle time analysis is a simple and insightful substitute for previously proposed more complex EDCA models.

==> previous.tex <==
\section{Previous Work}

A number of proposals were made to extend this Markov model for
the 802.11e EDCA function. \cite{Xiao05} includes the contention
window size differentiation in the EDCA mechanism, but lacks the
AIFS differentiation and the virtual collision scheme.
\cite{Robinson04} modifies the model by adding an in depth
treatment of the postcollision contention period, but the proposed
model remains complex. \cite{Tantra05} includes AIFS
differentiation for the two Access Category (AC) scenario, still
modelling the high priority AC as in \cite{Bianchi} which is not
correct. \cite{Kong04} provides a more complete model but misses
the handling collision probability differentiation for different
access categories after channel busy period finishes.

